Measurement of fiducial differential cross sections of gluon-fusion production of Higgs bosons decaying to $WW^{\ast}{\rightarrow\,}e\nu\mu\nu$ with the ATLAS detector at $\sqrt{s}=8$ TeV

This paper describes a measurement of fiducial and differential cross sections of gluon-fusion Higgs boson production in the $H{\rightarrow\,}WW^{\ast}{\rightarrow\,}e\nu\mu\nu$ channel, using 20.3 fb$^{-1}$ of proton-proton collision data. The data were produced at a centre-of-mass energy of $\sqrt{s} = 8$ TeV at the CERN Large Hadron Collider and recorded by the ATLAS detector in 2012. Cross sections are measured from the observed $H{\rightarrow\,}WW^{\ast}{\rightarrow\,}e\nu\mu\nu$ signal yield in categories distinguished by the number of associated jets. The total cross section is measured in a fiducial region defined by the kinematic properties of the charged leptons and neutrinos. Differential cross sections are reported as a function of the number of jets, the Higgs boson transverse momentum, the dilepton rapidity, and the transverse momentum of the leading jet. The jet-veto efficiency, or fraction of events with no jets above a given transverse momentum threshold, is also reported. All measurements are compared to QCD predictions from Monte Carlo generators and fixed-order calculations, and are in agreement with the Standard Model predictions.

==> tex/auxmat.tex <==
% !TEX spellcheck = en_UK
\section{Inputs to jet-veto efficiency}

In Table~\ref{tab:zerojet} the result for the fiducial cross section of $H+0$-jet events is given for the three different values of $\pT^{\mathrm{thresh}}$. 
\begin{table}[hbp!]
\centering
\caption{\label{tab:zerojet} Fiducial cross section of $H+0$-jet events in femtobarn for different values
 of $\pT^{\mathrm{thresh}}$ with the uncertainties for each bin given in absolute values and in percent. The asterisk for the $25\GeV$ column header
  indicates that the results are for a mixed $\pT$ threshold, which is raised from $25\GeV$ to $30\GeV$ for jets with $2.4<|\eta|<4.5$,
        corresponding to the selection used to define the signal regions for the analysis.} 
  \begin{tabular}{lrrr} 
  \dbline
  Jet $\pT$ threshold & $25\GeV$* & $30\GeV$ & $40\GeV$ \\ 
\sgline
$\sigma$~[fb]   & 19.0 & 20.7 & 23.3\\
    Statistical uncertainty              &  4.5 & 4.7 & 5.1 \\ 
    Total uncertainty                  &  6.8 & 7.1 & 8.2 \\
      \sgline
        SR data statistical        & 20\% & 19\% & 18\% \\
	MC statistical          &  4\% &  3\% &  3\% \\
	CR data statistical     & 12\% & 12\% & 12\% \\
	Exp. JER             &  5\% & 4\% & 5\% \\
	Exp. JES             &  1\% & 2\% & 5\% \\
	Exp. $b$-tag         &  1\% & 1\% & 2\% \\
	Exp. leptons    &  6\% & 6\% & 6\% \\
	Exp. $\MET$     &  2\% & 2\% & 2\% \\
	Exp. other      &  5\% & 6\% & 7\% \\
	Theory ($WW$)     & 24\% & 23\% & 22\% \\
	Theory (top)      & 2\% & 2\% & 4\% \\
	Theory (other backgrounds) & 5\% & 5\% & 6\% \\
	Theory (signal)   &  4\% & 5\% & 5\% \\
	Detector corrections    &  <1\% &  <1\% &  <1\% \\
	\sgline
	Total           &36\% & 34\% & 35\% \\
	  \dbline
	  \end{tabular}
	  \end{table}


\section{Correlation Matrices}

Bin-wise correlation matrices for the total uncertainty are given in Fig.~\ref{fig:corr_abs} for the measured
differential cross sections and in Fig.~\ref{fig:corr_norm} for the normalised measured differential cross sections.

\begin{figure}[!tbp]
  \centering
  \subfloat[$\Njet$]{
    \includegraphics[width=0.46\textwidth]{figures/corr/Njets_noOF_corr_statsys.pdf}

  }
  \subfloat[$\pTH$]{
    \includegraphics[width=0.46\textwidth]{figures/corr/PtllMET_vs_Njets_cutofftwo_corr_statsys.pdf}
  }
  \newline
  \subfloat[$\yll$]{
    \includegraphics[width=0.46\textwidth]{figures/corr/Yll_vs_Njets_cutofffour_corr_statsys.pdf}
  }
  \subfloat[$\pTj$]{
    \includegraphics[width=0.46\textwidth]{figures/corr/PtLeadJet_vs_Njets_cutofftwo_corr_statsys.pdf}
  }
  \caption{Full correlation matrices for the measured differential cross sections as a function of (a) $\Njet$, (b) $\pTH$, (c) $\yll$, and (d) $\pTj$ taking into account statistical and systematic uncertainties.   
    \label{fig:corr_abs}
    }
\end{figure}


\begin{figure}[!tbp]
  \centering
  \subfloat[$\Njet$]{
    \includegraphics[width=0.46\textwidth]{figures/corr/Njets_noOF_corr_statsys_norm.pdf}

  }
  \subfloat[$\pTH$]{
    \includegraphics[width=0.46\textwidth]{figures/corr/PtllMET_vs_Njets_cutofftwo_corr_statsys_norm.pdf}
  }
  \newline
  \subfloat[$\yll$]{
    \includegraphics[width=0.46\textwidth]{figures/corr/Yll_vs_Njets_cutofffour_corr_statsys_norm.pdf}
  }
  \subfloat[$\pTj$]{
    \includegraphics[width=0.46\textwidth]{figures/corr/PtLeadJet_vs_Njets_cutofftwo_corr_statsys_norm.pdf}
  }
  \caption{Full correlation matrices for the measured normalised differential cross sections as a function of (a) $\Njet$, (b) $\pTH$, (c) $\yll$, and (d) $\pTj$ taking into account statistical and systematic uncertainties.   
    \label{fig:corr_norm}
    }
\end{figure}

\section{Correction factors for parton-level predictions}

All parton-level predictions in this paper are corrected to particle level to allow comparison to data using the acceptance of the fiducial region and non-perturbative correction factors to account for the impact of hadronisation and underlying event activity. These factors are determined using {\POWHEG} {\NNLOPS}+\PythiaEight with the associated uncertainties from the renormalisation and factorisation scales as well as the PDFs. An uncertainty is assigned to the non-perturbative correction by comparing \PythiaEight with \HERWIG.

The parton-level predictions for the $\Njet$ distribution from BLPTW and for the $\pTj$ distribution from STWZ are fully inclusive except for the requirement that jets have $\pT > 25 \gev$ in case of BLPTW or $\pT > 30 \gev$ in case of STWZ. The correction factors for the predictions in each bin are given by the ratio of the default {\POWHEG} {\NNLOPS}+\PythiaEight prediction in the fiducial region over the fully inclusive {\POWHEG} {\NNLOPS}+\PythiaEight prediction with the requirements on the jets applied and the hadronisation and the underlying event in \PythiaEight turned off.
The factors are given in Table~\ref{tab:app_CF_njets} for the $\Njet$ prediction and in Table~\ref{tab:app_CF_pTj} for the $\pTj$ prediction.

\begin{table}[h]
\centering
\caption{ Correction factors from inclusive parton level to fiducial particle level for bins of $\Njet$ derived with {\POWHEG} {\NNLOPS}+\PythiaEight. Uncertainties due to the non-perturbative correction are dominant for the correction factors. }
\scalebox{0.95}{
\begin{tabular}{lccc}
\dbline
 & \ZeroJet & \OneJet & \TwoJet \\
   \sgline
  Correction factor 		& $0.0567^{+3.1\%}_{-2.6\%}$  	&  $0.0580^{+4.4\%}_{-4.5\%}$ &   $0.0628^{+6.3\%}_{-6.7\%}$  \\	
 \dbline
\end{tabular}}
\label{tab:app_CF_njets}
\end{table}

\begin{table}[h]
\centering
\caption{ Correction factors from inclusive parton level to fiducial particle level for bins of $\pTj$ derived with {\POWHEG} {\NNLOPS}+\PythiaEight. Uncertainties due to the non-perturbative correction are dominant for the correction factors.}
\scalebox{0.95}{
\begin{tabular}{lccc}
\dbline
 \pTj & $[0, 30] \gev$ & $[30, 60] \gev$ & $[60, 300] \gev$ \\
   \sgline
  Correction factor 		& $0.0551^{+3.0\%}_{-2.7\%}$  	&  $0.0569^{+5.5\%}_{-5.5\%}$ &   $0.0718^{+7.0\%}_{-7.0\%}$  \\	
 \dbline
\end{tabular}}
\label{tab:app_CF_pTj}
\end{table}

The parton-level predictions for the jet-veto efficiency $\varepsilon_{0}$ from the ST, JetVHeto, STWZ, and\linebreak N$^{3}$LO+NNLL+LL\_R are again calculated in the inclusive phase space. For the predictions of the jet-veto efficiency for the jet selection used in the analysis, $25\GeV$ for central jets ($|\eta|<2.4$) and $30\GeV$ for forward jets ($2.4<|\eta|<4.5$), the inclusive parton-level predictions with $\pTj > 25 \gev$ are used. For the $30\GeV$ and $40\GeV$ thresholds in the efficiency 
calculation the correction accounts for the restriction of jets to $|\eta|<4.5$.
All correction factors and their uncertainties are given in Table~\ref{tab:app_CF_JV}. 

\begin{table}[h]
\centering
\caption{ Correction factors from inclusive parton level to fiducial particle level for the jet-veto efficiency with different jet $\pT$ thresholds derived with {\POWHEG} {\NNLOPS}+\PythiaEight. The asterisk on the $25\GeV$ bin label indicates that the results are for a mixed $\pT$ threshold, which is raised from 
    $25\GeV$ to $30\GeV$ for jets with $2.4<|\eta|<4.5$, corresponding to the selection used to define the signal regions for the analysis. }
\scalebox{0.95}{
\begin{tabular}{lccc}
\dbline
 jet $\pT$ threshold & $25\GeV$* & $30\GeV$ & $40\GeV$ \\
   \sgline
  Correction factor inclusive 		& $0.9798^{+1.2\%}_{-0.3\%}$  	&  $0.9529^{+1.0\%}_{-0.5\%}$ &   $0.9534^{+1.0\%}_{-0.5\%}$  \\	
 \dbline
\end{tabular}}
\label{tab:app_CF_JV}
\end{table}

\section{Control Region Distributions}

In this section all control-region distributions are presented for the $\pTH$, $\pTj$, and $\yll$ distributions that are not included in the main part of this paper.
In Fig.~\ref{fig:WWCRaux} the $\pTH$ distribution is shown in the $\ZeroJet$ $WW$ control region, and the $\yll$ and \pTj distributions are shown in the $\OneJet$ $WW$ control region.
Figure~\ref{fig:TopCRaux} gives $\pTH$ and $\yll$ distributions in the $\OneJet$ top-quark control region and the $\pTj$ and $\yll$ distributions in the $\TwoJet$ top-quark control region. The $\pTH$ distribution in the $\ZeroJet$ same-sign control region and the $\pTH$, $\pTj$, and $\yll$ distributions in the $\OneJet$ same-sign control region are given in Fig.~\ref{fig:SSCRaux}.
The remaining distributions in the $\Ztt$ control regions are presented in Fig.~\ref{fig:ZttCRaux}: $\yll$ in the $\ZeroJet$ and $\OneJet$, $\pTj$
in the $\OneJet$ and $\TwoJet$, and $\pTH$ in the $\ZeroJet$ control regions.
 
 
\begin{figure}[ptb]
  \centering
  \subfloat[$\pTH$, $\ZeroJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutWWControl_0jet_PtllMET.pdf}
  }
  \subfloat[$\yll$, $\OneJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutWWControl_1jet_Yll.pdf}
  }
  \newline
  \subfloat[$\pTj$, $\OneJet$]{
    \includegraphics[width=0.40\textwidth]{auxiliary/all_CutWWControl_1jet_PtLeadJet.pdf}
  }
  \caption{ \label{fig:WWCRaux}  Observed distributions of (a) $\pTH$ in the $\ZeroJet$, (b) $\yll$ in the $\OneJet$ , and (c) $\pTj$ 
      in the $\OneJet$ $WW$ control regions, with signal and background expectations.  
	Relevant background normalisation factors have been applied.
	The small predicted contribution from the SM Higgs boson is summed over all production processes.
      The hatched band in the upper panel and the shaded band in the lower panel show the sum in quadrature of statistical 
    and systematic uncertainties of the prediction. 
    }
\end{figure}

\begin{figure}[ptb]
  \centering
  \subfloat[$\pTH$, $\OneJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutTopControl_1jet_PtllMET.pdf}
  }
  \subfloat[$\pTj$, $\TwoJet$]{
    \includegraphics[width=0.40\textwidth]{auxiliary/all_CutFailVBFHighMllTopCR_2jetincl_PtLeadJet.pdf}
  }
  \newline
  \subfloat[$\yll$, $\OneJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutTopControl_1jet_Yll.pdf}
  }
  \subfloat[$\yll$, $\TwoJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutFailVBFHighMllTopCR_2jetincl_Yll.pdf}
  }

  \caption{ \label{fig:TopCRaux}  Observed distributions of (a) $\pTH$ in the $\OneJet$, (b) $\pTj$ in the $\TwoJet$, and (c, d) $\yll$  
      in the (c) $\OneJet$ and (d) $\TwoJet$ top-quark control regions, with signal and background expectations.  
	Relevant background normalisation factors have been applied.
	The small predicted contribution from the SM Higgs boson is summed over all production processes.
      The hatched band in the upper panel and the shaded band in the lower panel show the sum in quadrature of statistical 
    and systematic uncertainties of the prediction.
    }
\end{figure}

\begin{figure}[ptb]
  \centering
  \subfloat[$\pTH$, $\ZeroJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutFRecoil_0jet_sscr_PtllMET.pdf}
  }
  \subfloat[$\pTH$, $\OneJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutFRecoil_1jet_sscr_PtllMET.pdf}
  }
  \newline
  \subfloat[$\yll$, $\OneJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutFRecoil_1jet_sscr_Yll.pdf}
  }
  \subfloat[$\pTj$, $\OneJet$]{
    \includegraphics[width=0.40\textwidth]{auxiliary/all_CutFRecoil_1jet_sscr_PtLeadJet.pdf}
  }
  \caption{ \label{fig:SSCRaux}  Observed distributions of (a, b) $\pTH$, (c) $\yll$, and (d) $\pTj$ 
      in the (a) $\ZeroJet$ and (b, c, d) $\OneJet$ same-sign control regions, with signal and background expectations.  
	Relevant background normalisation factors have been applied.
	The small predicted contribution from the SM Higgs boson is summed over all production processes.
      The hatched band in the upper panel and the shaded band in the lower panel show the sum in quadrature of statistical 
    and systematic uncertainties of the prediction.
    }
\end{figure}

\begin{figure}[ptb]
  \centering
  \subfloat[$\yll$, $\ZeroJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutZttControl_0jet_Yll.pdf}
  }
  \subfloat[$\yll$, $\OneJet$]{
 	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutZttControl_1jet_Yll.pdf}
  }
  \newline
  \subfloat[$\pTj$, $\OneJet$]{
    \includegraphics[width=0.40\textwidth]{auxiliary/all_CutZttControl_1jet_PtLeadJet.pdf}
  }
  \subfloat[$\pTj$, $\TwoJet$]{
    \includegraphics[width=0.40\textwidth]{auxiliary/all_CutZtautauControl_2jetincl_PtLeadJet.pdf}
  }
  \newline
  \subfloat[$\pTH$, $\ZeroJet$]{
	\includegraphics[width=0.40\textwidth]{auxiliary/all_CutZttControl_0jet_PtllMET.pdf}
  }

  \caption{ \label{fig:ZttCRaux}  Observed distributions of (a, b) $\yll$, (c, d) $\pTj$, and (e) $\pTH$
      in the (c, e) $\ZeroJet$, (b,c) $\OneJet$, and (d) $\TwoJet$ $\Ztt$ control regions, with signal and background expectations.  
	Relevant background normalisation factors have been applied.
	The small predicted contribution from the SM Higgs boson is summed over all production processes.
      The hatched band in the upper panel and the shaded band in the lower panel show the sum in quadrature of statistical 
    and systematic uncertainties of the prediction.
    }
\end{figure}

\section{Signal region distributions, log scale}

Figure~\ref{fig:measureddistributionsAUX} shows the distributions to be unfolded in the signal region, prior to unfolding, 
  summed over $\Njet$.  These are identical to Fig.~\ref{fig:measureddistributions} but with the upper panel in log scale.

\begin{figure}[!tbp]
  \centering
  \subfloat[$\Njet$]{
    \includegraphics[width=0.46\textwidth]{auxiliary/Njets_log.pdf}
  }
  \subfloat[$\pTH$]{
    \includegraphics[width=0.46\textwidth]{auxiliary/PtllMET_log.pdf}
  }
  \newline
  \subfloat[$\yll$]{
    \includegraphics[width=0.46\textwidth]{auxiliary/Yll_log.pdf}
  }
  \subfloat[$\pTj$]{
    \includegraphics[width=0.46\textwidth]{auxiliary/PtLeadJet_log.pdf}
  }
  \caption{Observed distributions of (a) $\Njet$, (b) $\pTH$, (c) $\yll$, and (d) $\pTj$ with signal and background expectations, combined 
    over the \AllJet\ signal-region categories.   The background processes are normalised as described in Section~\ref{sec:background}.  
		  The SM Higgs boson signal prediction shown is summed over all production processes.
In the $\pTj$ distribution, $\ZeroJet$ events are all in the first bin by construction because of the definition of the jet thresholds used
to define the signal regions.
  The hatched band shows the sum in quadrature of statistical and systematic uncertainties of the sum of the backgrounds. 
  \label{fig:measureddistributionsAUX}
    }
\end{figure}


